Sequence Modeling with Unconstrained Generation Order

The dominant approach to sequence generation is to produce a sequence in some predefined order, e.g. left to right. In contrast, we propose a more general model that can generate the output sequence by inserting tokens in any arbitrary order. Our model learns decoding order as a result of its training procedure. Our experiments show that this model is superior to fixed order models on a number of sequence generation tasks, such as Machine Translation, Image-to-LaTeX and Image Captioning.

==> experiments.tex <==







\section{Results}
%\subsection{Machine Translation}\label{sect:mt}
\input{main_table.tex}

%НАДОСКАЗАТЬ:
%* что-то про порядок слов в языках
%* процитировать Aspec, остальные как в https://arxiv.org/abs/1809.00120
%* we use the original Transformer base + nlda + large batch \cite{training_tips_transformer}. There are possible improvements (e.g. label smoothing, backtranslation) but those are equally applicable to both models.
%* В частности, \cite{checkpoint_averaging}, \cite{label_smoothing}, \cite{dual_learning} и вообще \cite{combining_hacks}
%* training speed, inference complexity
%\subsection{Image-to-Sequence experiments}
%As an additional proof of concept, we evaluate on two more sequence generation problems, but with an image as the model input. Table \ref{tab:main} demonstrates that our model outperforms fixed order baselines on image to sequence tasks.


Table \ref{tab:main} demonstrates that our model outperforms fixed order baselines on the selected tasks.

% \begin{table}[h!]
% \small
% \centering
% \renewcommand\arraystretch{1.3}

% \vspace{-3mm}
% \caption{Image-to-Sequence experiments.}

% \begin{tabular}{|c|c|c|c|}

% \hline
% Model &    Im2Latex  & \multicolumn{2}{|c|}{MSCOCO} \\
% \cline{2-4}
%       & Token BLEU   &  BLEU  & CIDEr   \\
% \hline
% Left-to-right   &   89.5   &  18    & 0.56 \\ 
% \citet{Im2latex2} &   89.0   &    -  & - \\
% Ours            &   \textbf{90.3}   & \textbf{25.6} & \textbf{0.81}  \\ 
% \hline
% \end{tabular}
% \label{tab:image}
% \end{table}

\subsection{Ablation analysis} \label{sect:ablation}
This section empirically validates the training and inference strategies proposed in Section \ref{sect:method}. We begin by comparing the following training strategies on WMT English-Russian translation task using development set (2012-2013 WMT test sets) in table \ref{tab:ablation_training}:

\begin{itemize}[leftmargin=2mm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
\itemsep-0.1em
    \item \textbf{Ours} - the training procedure as described in  Section \ref{sec::experiements}.
    \item \textbf{Argmax} - alternative training procedure used in the concurrent study by \citet{Gu2019InsertionbasedDW}. This procedure always trains the model on the most likely trajectory in $T^*(Y)$ that can be found using beam search (size 4).
    \item \textbf{Pretrain left-to-right} - like Ours, but pretraining is conducted not with uniform samples, but with the fixed left-to-right decoding order.
    \item \textbf{Only pretraining} - training is performed with a model-independent order, either uniform or left-to-right. This strategy is similar to \citet{Stern2019InsertionTF}.
\end{itemize}
\begin{table*}[h!]
\vspace{-1mm}
 \centering
\caption{Training strategies on EN-RU translation task}
\begin{tabular}{c c c c c c c c }
     \toprule
     %\hline
     Training & \multirow{2}{*}{Ours} & \multirow{2}{*}{Argmax} & Pretraining & No pre- & \multicolumn{2}{c}{Only pretraining} & Baseline \\
     \cmidrule{6-7}
     strategy & & & left-to-right & training & uniform & left-to-right & left-to-right \\
     \midrule
     BLEU & 27.5 & 26.6 & 26.3 & 27.1 & 24.6 & 25.5 & 25.8 \\
     \bottomrule

\end{tabular}
\label{tab:ablation_training}
\vspace{-3mm}
\end{table*}
\subsection{Stability and Complexity}

This process, however, is rather slow. During early stages of training, we sample trajectories uniformly from $T^*(Y)$. \lena{maybe say why pretraining} Such sampling is much faster, as it does not require inference from the model at each training step.
%\cite{order_matters} employed the same trick in their work. 
For both our model and all baselines, we update $\theta$ using Adam \cite{kingma2014adam} with a transformer learning rate schedule \cite{transformer,smith2017super}, similar to the one used in the original Transformer.

\paragraph{Stability} An important observation from our experiments is that introducing any of the two pretraining strategies greatly increases the overall robustness of our training procedure and avoids premature convergence to local optima that can be observed in the experiments that lack pretraining. We attribute this to the fact that a pretrained model establishes a good initial policy for the main algorithm. The Argmax training strategy, while starting from a good pretrained model, tends to quickly converge to the current best trajectory which may not be globally optimal. This training mode produces less stable results and is the only strategy that required several consecutive runs to obtain reasonable quality.

\paragraph{Computational complexity} The training procedure described in Section \ref{sect:method} is more computationally expensive than that of the conventional transformer. While the exact numbers vary from one dataset to another, on average INTRUS trains 3-4 times as long as the baseline. As for the inference, theoretical computational complexity of beam search is $O(|Y|^3 k)$ compared to $O(|Y|^2k)$ complexity of conventional left-to-right models. Empirically, however,  despite our model performing up to 4 times slower on long input sequences, it translates a typical dataset only $50\%$ slower due to most sentences being short (see Figure \ref{fig::complexity}).

\begin{figure}[h]
    \vspace{-7pt}
    
    \begin{minipage}{0.43\textwidth}
        \centering
        \includegraphics[width=160pt]{resources/complexity.png}
        \caption{Inference time of our and baseline models and sentence length distribution.}
        \label{fig::complexity}
        %\centering
        % \captionsetup{type=table} %% tell latex to change to table
        % \caption{Training strategies on EN-RU translation task}
        % \begin{tabular}{|c|c|}
        %      \hline
        %      Training strategy & BLEU \\
        %      \hline
        %      Ours & \textbf{27.5}\\
        %      Argmax & 26.6\\
        %      Pretrain left-to-right & 26.3\\
        %      No pretraining & 27.1\\
        %      Only pretraining (uniform)  & 24.6\\
        %      Only pretraining (left-to-right)  & 25.5\\
        %      Baseline (left-to-right) & 25.8\\
        %      \hline
        % \end{tabular}
        % \vspace{-2ex}
        % \label{tab:ablation_training}
    \end{minipage}
    \hfill
    \begin{minipage}{0.55\textwidth}
        \centering
        \includegraphics[width=220pt]{resources/inversions_cropped.png}
        \caption{The distributions of fractions of leaf and non-leaf dependency inversions in each sentence.}
        \label{fig::inversions}
    \end{minipage}
\end{figure}

